The Complexity of Counting Edge Colorings for Simple Graphs

We prove #P-completeness results for counting edge colorings on simple graphs. These strengthen the corresponding results on multigraphs from [4]. We prove that for any $\kappa \ge r \ge 3$ counting $\kappa$-edge colorings on $r$-regular simple graphs is #P-complete. Furthermore, we show that for planar $r$-regular simple graphs where $r \in \{3, 4, 5\}$ counting edge colorings with \k{appa} colors for any $\kappa \ge r$ is also #P-complete. As there are no planar $r$-regular simple graphs for any $r > 5$, these statements cover all interesting cases in terms of the parameters $(\kappa, r)$.

==> bibliography.tex <==
\begin{thebibliography}{50}
\bibitem{Berman-Hartmanis}
Leonard Berman, Juris Hartmanis: On Isomorphisms and Density of NP and Other Complete Sets. SIAM J. Comput. 6(2): 305-322 (1977).

\bibitem{Blass-Gurevich}
Andreas Blass and Yuri Gurevich: On the unique satisfiability problem. Information and Control.
Volume 55, Issues 1-3, October-December 1982, Pages 80-88.

\bibitem{cai-chen-book}
Jin-Yi Cai and Xi Chen: {\it Complexity Dichotomies for Counting Problems}, Volume 1: Boolean Domain,
 Cambridge University Press, 2017.
\url{https://doi.org/10.1017/9781107477063}.
%\href{https://doi.org/10.1017/9781107477063}{https://doi.org/10.1017/9781107477063}.

\bibitem{cgw-focs-2014}
Jin-Yi Cai, Heng Guo, Tyson Williams:
The Complexity of Counting Edge Colorings and a Dichotomy for Some Higher Domain Holant Problems.
Research in the Mathematical Sciences,
(2016) 3:18.
A preliminary version in FOCS 2014: 601-610.

\bibitem{Diestel-book} %to edit
%Diestel, Reinhard (2000), Graph Theory (PDF), Berlin, New York: Springer-Verlag, pp. 103-104.
%Reinhard Diestel:
%Graph Theory, 4th Edition. Graduate texts in mathematics 173, Springer 2012, ISBN 978-3-642-14278-9, pp. I-XVIII, 1-436
%%%
%Springer-Verlag, Heidelberg
%Graduate Texts in Mathematics, Volume 173
%ISBN 978-3-662-53621-6   eISBN 978-3-96134-005-7
%August 2016 (2010, 2005, 2000, 1997)
%447 pages; 124 figures
%%%
R. Diestel: Graph Theory, 5th Edition. Graduate Texts in Mathematics 173, Springer 2016. %, ISBN 978-3-662-53621-6, 447 pages. %August 2016 %978-3-662-53621-6 %Reinhard Diestel

\bibitem{Edwards-Welsh} K. J. Edwards and D. J. A. Welsh:
On the complexity of uniqueness problems (unpublished) (1983).

\bibitem{Hol81}
%Ian Holyer. The NP-completeness of edge-coloring. SIAM J. Comput., 10(4):718-720, 1981. %bib
I. Holyer: The NP-completeness of edge-coloring. SIAM J. Comput. 10(4), 718-720 (1981). %I. Holyer

\bibitem{Isaacs-1975}
R. Isaacs: Infinite families of nontrivial trivalent graphs which are not Tait colorable, Amer. Math. Monthly, 82 (1975), pp. 221-239. %Rufus Isaacs

\bibitem{LG83}
%Daniel Leven and Zvi Galil. NP completeness of finding the chromatic index of regular graphs. J. Algorithm., 4(1):35-44, 1983. %bib
D. Leven, Z. Galil: NP completeness of finding the chromatic index of regular graphs. J. Algorithm 4(1), 35-44 (1983). %Leven, D., Galil, Z.

\bibitem{JanosSimon} %1977 ICALP 480-491
Janos Simon: On the Difference Between One and Many (Preliminary Version). ICALP 1977: 480-491.

%\bibitem{SSTF12}
%M. Stiebitz, D. Scheide, B. Toft, L.M. Favrholdt: Graph Edge Coloring: Vizing's Theorem and Goldberg's Conjecture.
%Wiley, New York (2012). %Stiebitz, M., Scheide, D., Toft, B., Favrholdt, L.M.

\bibitem{Tai80}
%Peter Tait. Remarks on the colourings of maps. Proc. R. Soc. Edinburgh, 10:729, 1880. %bib
P. Tait: Remarks on the colourings of maps. Proc. R. Soc. Edinb. 10, 729 (1880). %Tait, P.

\bibitem{Thomason1978}
%A. G. Thomason. Hamiltonian cycles and uniquely edge colourable
%graphs, Advances in Graph Theory (Cambridge Combinatorial Conf.,
%Trinity College, Cambridge, 1977), Annals of Discrete Mathematics, 3,
%pp. 259-268, 1978.
A. G. Thomason: Hamiltonian cycles and uniquely edge colourable graphs.
Annals of Discrete Mathematics 3 (1978) pp. 259-268. %Andrew Gordon Thomason.

\bibitem{Viz65}
%Vadim G. Vizing. Critical graphs with given chromatic class. Metody Diskret. Analiz., 5:9-17, 1965. %bib
V. G. Vizing: Critical graphs with given chromatic class. Metody Diskret. Analiz. 5, 9-17 (1965). %Vizing, V.G.

\bibitem{Wel93}
%Dominic Welsh. Complexity: Knots, Colourings and Countings. London Mathematical Society Lecture Note Series. Cambridge University Press, 1993. %bib
D. J. A. Welsh:
Complexity: Knots, Colourings and Countings (London Mathematical Society Lecture Note Series) %% Cambridge University Press; 1 edition (August 27, 1993)
Cambridge University Press; 1st edition (August 27, 1993).

% \bibitem{JanosSimon} 1977 ICALP 480-491
%Janos Simon:
%On the Difference Between One and Many (Preliminary Version). ICALP 1977: 480-491
%\bibitem{Berman-Hartmanis}
%Leonard Berman, Juris Hartmanis:
%On Isomorphisms and Density of NP and Other Complete Sets. SIAM J. Comput. 6(2): 305-322 (1977)
%\bibitem{Valiant-unpublished}
%Les Valiant: A reduction from satisfiability to Hamiltonian circuits that
% preserves the number of solutions, Unpublished manuscript, Leeds, 1974.

% \bibitem{Wel93} 
%%% 	D. J. A. Welsh
%Complexity: Knots, Colourings and Countings (London Mathematical Society Lecture Note Series) %% Cambridge University Press; 1 edition (August 27, 1993) %%
%%
%% \bibitem{Edwards-Welsh} K. J. Edwards and D. J. A. Welsh
%% On the complexity of uniqueness problems (unpublished). (1983).
%%
%% \bibitem{Blass-Gurevich}  Andreas Blass and Yuri Gurevich
%% On the unique satisfiability problem
%  Information and Control
%Volume 55, Issues 1-3, October-December 1982, Pages 80-88
%%
%%%%%%% also cite the following
%{\bf Witness-Isomorphic Reductions and Local Search},
%S.~Fischer, L.~Hemaspaandra, and L.~Torenvliet,
%in~\uline{Complexity, Logic and Recursion Theory},
%ed.~A.~Sorbi, Marcel Dekker, Inc., pp.~207--223,
%1997.
%%%%%%%
\end{thebibliography}

==> his-preamble.tex <==
%\documentclass[11pt,twoside]{article}
\usepackage{amsmath, amsfonts, amssymb, amsthm, amscd, graphicx, 
%hyperref, 
enumerate, footmisc, mathtools, xcolor}
\setcounter{MaxMatrixCols}{30}
\setcounter{tocdepth}{10}
\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
\setlength{\topmargin}{-1.0in}
\setlength{\textheight}{9.25in}
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in}
\setlength{\textwidth}{6.5in}
\def\labelenumi{\arabic{enumi}.}
\def\theenumi{\arabic{enumi}}
\def\labelenumii{(\alph{enumii})}
\def\theenumii{\alph{enumii}}
\def\p@enumii{\theenumi.}
\def\labelenumiii{\arabic{enumiii}.}
\def\theenumiii{\arabic{enumiii}}
\def\p@enumiii{(\theenumi)(\theenumii)}
\def\labelenumiv{\arabic{enumiv}.}
\def\theenumiv{\arabic{enumiv}}
\def\p@enumiv{\p@enumiii.\theenumiii}
\pagestyle{plain}
%\parindent=0pt
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}{Remark}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{axiom}{Axiom}

\newenvironment{lcases}
  {\left\lbrace\begin{aligned}}
  {\end{aligned}\right.}
\newcommand{\bbF}{\mathbb F}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbC}{\mathbb C}
\newcommand{\bbH}{\mathbb H}
\newcommand{\pmatch}{\operatorname{pm}}
\newcommand{\edgecol}{\operatorname{ec}}
\newcommand{\vdccover}{\operatorname{vdcc}}
\newcommand{\wmatch}{\operatorname{wm}}
\newcommand{\Char}{\operatorname{char}}
\newcommand{\Mod}{\operatorname{mod}}
%\newcommand{\rank}{\operatorname{rk}}
\newcommand{\symrank}{\operatorname{rk_\mathsf S}}
\newcommand{\matrank}{\operatorname{rank}}
\newcommand{\im}{\operatorname{im}}
%\newcommand{\Holant}{\operatorname{Holant}}
%\newcommand{\trans}[4]{\ensuremath{\left[ \begin{smallmatrix} #1 & #2 \\ #3 & #4 \end{smallmatrix} \right]}}
\newcommand{\Span}{\operatorname{span}}
%\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\id}{\operatorname{id}}
%\newcommand{\diag}{\operatorname{diag}}
%\newcommand{\dom}{\operatorname{dom}}

\newcommand{\calPLG}{\mathcal{PLG}}
\newcommand{\calG}{\mathcal G}
\newcommand{\calK}{\mathcal K}
\newcommand{\calP}{\mathcal P}
\newcommand{\bfx}{\mathbf x}
\newcommand{\bfy}{\mathbf y}
\newcommand{\bfz}{\mathbf z}
\newcommand{\sfS}{\mathsf S}
\newcommand{\sfT}{\mathsf T}
\newcommand{\calM}{\mathcal M}
\newcommand{\bfu}{\mathbf u}
\newcommand{\bfv}{\mathbf v}
\newcommand{\bff}{\mathbf f}
\newcommand{\textbfit}[1]{\textbf{\textit{#1}}}
\newcommand{\calI}{\mathcal I}
\newcommand{\calJ}{\mathcal J}
\newcommand{\calA}{\mathcal A}
\newcommand{\calT}{\mathcal T}

\newcommand*{\mainflag}{}



==> interpolation-argument.tex <==
{\color{red} interpolation argument}
\newcommand{\EVAL}{\operatorname{EVAL}}

%\section{Hardness for $Z_A(\cdot)$ on simple graphs for real symmetric $A$}
%
%There is a more direct approach to prove 
%the \#P-hardness part of the Bulatov-Grohe dichotomy
%(Theorem~\ref{thm:Bulatov-Grohe}) for  simple graphs.
%Although this method does not handle degree-boundedness,
%we can apply it more generally to the problem $\EVAL(A, D)$
%when the matrix $A$ is real symmetric
%and $D$ is positive diagonal,
%as long as there is a corresponding dichotomy for counting GH.
%In particular, we will prove 
%the \#P-hardness part of the dichotomy for counting GH
%by Goldberg et al.~\cite{Goldberg-et-al-2010} (the problem $\EVAL(A)$ 
%without vertex weights, where $A$ is a real symmetric matrix)
%for  simple graphs.
%
%We first prove the following theorem.
%\begin{theorem}\label{thm:EVAL-simp-interp}
%Let $A$ and $D$ be $m \times m$ matrices,
%where $A$ is real symmetric and $D$ is positive diagonal.
%Then $\EVAL(A, D) \le_{\mathrm T}^{\mathrm P} \EVAL_{\simp}(A, D)$.
%\end{theorem}

%\begin{proof}
%We may assume $A$ is not identically $0$, for otherwise the problem is
%trivial.
%Let $G = (V, E)$ be an input graph to the problem $\EVAL(A, D)$.
%For any $n \ge 1$, let $G_n = S_n^{(F)}(G)$ where $F \subseteq E$ is the
%subset consisting of the edges of $G$ each of which is parallel 
%to at least one other edge. 
%In other words, we obtain $G_n$ by replacing every parallel edge $e$
%by its $n$-stretching $S_n e$.
%%{\color{red} In other words, we define $G_n$ as a modification on $G$
%%by stretching every parallel edge in $G$:
%%each parallel edge $e$ is replaced by $S_n e$.}
%We will refer to these as paths of length $n$ in $G_n$.
%Note that $G_1 = G$.
%Moreover, for every $n \ge 2$, the graph $G_n$ is simple and loopless,
%and has polynomial size in the size of $G$ and $n$.
%%{\color{red} copied interpolation argument from main proof and changed accordingly}
%
%A path of length $n \ge 1$ has the edge weight matrix
%\[
%M^{(n)}=
%\underbrace{A D A \ldots A D A}_{D \text{ appears } n - 1 ~\ge~ 0 \text{ times}} = A (D A)^{n - 1} = D^{-1 / 2} (D^{1 / 2} A D^{1 / 2})^n D^{-1 / 2}.
%\]
%Here $D^{1 / 2}$ is a diagonal matrix
%with the positive square roots
%of the corresponding entries
%of $D$ on the main diagonal,
%and $D^{-1 / 2}$ is its inverse.

Since $A$ is real symmetric and $D$ is positive diagonal,
the matrix $\widetilde A = D^{1 / 2} A D^{1 / 2}$ is real symmetric.
Then $\widetilde A$ is orthogonally diagonalizable over $\mathbb{R}$, i.e.,
there exist a real orthogonal matrix $S$
and a real diagonal matrix $J = (\lambda_i)_{i = 1}^m$ such that $\widetilde A = S^T J S$.
If $A$ has rank $r$, then $1 \le r \le m$,
and we may assume
that $\lambda_i \ne 0$ for $1 \le i \le r$
and $\lambda_i = 0$ for $i > r$.
%%% correction from Artem: I should not make the following statement,
%%% but carry on with 1 to m for indexing of M^{(n)}
%
%Clearly the problems 
% $\EVAL(A, D)$ and $\EVAL_{\simp}(A, D)$ are equivalent
%to the same problem defined on the domain set $[r]$.
%%%% for isolated vertices get a factor d_1 + ... d_m > 0.
%%%% then for any other component, kill off d_{>r}.
%%%% 
%Therefore we may assume $r=m$.
 
%Then 
We have ${\widetilde A}^n = S^T J^n S$, so the edge weight matrix for a path of length $n \ge 1$ can be written as 
\[
M^{(n)} 
%= A (D A)^{n - 1} 
= D^{-1 / 2} {\widetilde A}^n D^{-1 / 2}
= D^{-1 / 2} S^T J^n S D^{-1 / 2}.
\]

We can write $M_{i j}^{(n)} = \sum_{\ell = 1}^r a_{i j \ell} \lambda_\ell^n$
by a formal  expansion,
for every $n \ge 1$ and some real $a_{i j \ell}$'s
that are dependent on $D$ and $S$, but independent of $n$ and $\lambda_\ell$,
where $1 \le i, j \le m$ and $1 \le \ell \le r$. 
%%% JYC I don't think it is necessary to remark this symmetry
% which we can arrange, and would be do if by "formnal expansion
% but not necessarily true if just by "such an expression as linear comb.
%
% Since $M^{(n)}$
%is symmetric, by the formal  expansion we have $a_{i j \ell} = a_{j i \ell}$.
%
%%%
By the formal expansion of the symmetric matrix $M^{(n)}$ above,
we have $a_{i j \ell} = a_{j i \ell}$.
%%%
Let $t = |F|$, which is the number of edges in $G$
subject to the stretching operator $S_n$ to form $G_n$.

In the evaluation of the partition function $Z_{A, D}(G_n)$,
we stratify the vertex assignments in $G_n$ as follows.
Denote by  $\kappa = (k_{i j})_{1 \le i \le j \le m}$
a nonnegative tuple with entries indexed by ordered pairs of numbers
and satisfy $\sum_{1 \le i \le j \le m} k_{i j} = t$.
Let $c_\kappa$ 
be the sum over all assignments of all vertex and edge weight products
in $Z_{A, D}(G_n)$,
 except the contributions by the paths of length $n$ formed by
stretching parallel edges in $G$,
such that the endpoints of precisely $k_{i j}$ constituent paths
 of length $n$
receive the assignments $(i, j)$ (in either order of the end points)
 for every $1 \le i \le j \le m$.
Let $\mathcal K$ denote the set of all such possible tuples $\kappa$.
In particular, $|\mathcal K| = \binom{t + m (m + 1) / 2 - 1}{m (m + 1) / 2 - 1}$.
Then
\[
Z_{A, D}(G_n) = \sum_{\kappa \in \mathcal K} c_\kappa \prod_{1 \le i \le j \le m} (M_{i j}^{(n)})^{k_{i j}}
= \sum_{\kappa \in \mathcal K} c_\kappa \prod_{1 \le i \le j \le m} (\sum_{\ell = 1}^r a_{i j \ell} \lambda_\ell^n)^{k_{i j}}. 
\]
%Note that $(M^{(n)})_{i j} = (M^{(n)})_{j i}$ so everything is well-defined.
Expanding out the last sum and rearranging the terms we get
\begin{equation}\label{interpolation-lin-sys-sec4}
Z_{A, D}(G_n)
= \sum_{\substack{i_1 + \ldots + i_r = t \\ i_1, \ldots, i_r \ge 0}} b_{i_1, \ldots, i_r} ( \prod_{\ell = 1}^r \lambda_\ell^{i_\ell} )^n.
\end{equation}

This can be viewed as a linear system with the unknowns $b_{i_1, \ldots, i_r}$ with the rows indexed by $n$. % Vandermonde
The number of unknowns is  $\binom{t + r - 1}{r - 1}$
which is polynomial in the size of the input graph $G$, since $r \le m$ is a constant.
So the number of unknowns is 
polynomial in the size of the input graph $G$.
The values $\prod_{\ell = 1}^r \lambda_\ell^{i_\ell}$
can all be computed in polynomial time.

We show how to compute the value $Z_{A, D}(G) = \displaystyle \sum_{\scriptsize \substack{i_1 + \ldots + i_r = t \\ i_1, \ldots, i_r \ge 0}} b_{i_1, \ldots, i_r} \prod_{\ell = 1}^r \lambda_\ell^{i_\ell}$,
from the values $Z_{A, D}(G_n)$ where $n \ge 2$ in polynomial time
(recall that $G_n$ is simple and loopless for $n \ge 2$).
The coefficient matrix of the linear system (\ref{interpolation-lin-sys-sec4})
 is Vandermonde.
However, it might not be of full rank
because the coefficients $\prod_{\ell = 1}^r \lambda_\ell^{i_\ell}$
do not have to be pairwise distinct, and therefore
it can have repeating columns.
Nevertheless, when there are two repeating columns we replace
the corresponding unknowns $b_{i_1, \ldots, i_r}$ and $b_{i'_1, \ldots, i'_r}$
with their sum as a new variable; we repeat this replacement procedure until
there are no repeating columns.
Since all $\lambda_\ell \ne 0$, for $1 \le \ell \le r$,
after the replacement,
 we have a Vandermonde system of full rank.
% after all such combinations.
Therefore we can solve this modified linear system
in polynomial time.
This allows us to obtain the value $Z_{A, D}(G) = \displaystyle \sum_{\substack{i_1 + \ldots + i_r = t \\ i_1, \ldots, i_r \ge 0}} b_{i_1, \ldots, i_r} \prod_{\ell = 1}^r \lambda_\ell^{i_\ell}$, which also has exactly the same pattern of repeating multipliers
$\prod_{\ell = 1}^r \lambda_\ell^{i_\ell}$. 
%More precisely, we only need the value of $Z_{A, D}$ on the instances $G_{n, p}$ where $2 \le n \le \ell + 1$
%where $\ell \le \binom{t + m - 1}{m - 1}$ is the number of distinct numbers $\prod_{j = 1}^m \lambda_j^{i_j}$,
%(so there are polynomial many of them and each is of the size
%polynomially bounded in the size of $G$).

%We have shown how to compute the value $Z_{A, D}(G)$ in polynomial time
%by querying  the oracle $\EVAL(A, D)$ 
%on polynomially many instances $G_n$, for $n \ge 2$.
%%where $2 \le p \le \ell + 1$ 
%%in polynomial time.
%It follows that $\EVAL(A, D) \le_{\mathrm T}^{\mathrm P} \EVAL_{\simp}(A, D)$.
%\end{proof}

%{\color{red} removed first sentence and changed lemma to theorem \ref{thm:EVAL-simp-interp} everywhere including below remark}

%This completes the proof for our reduction to $\EVAL_{\simp}(A, D)$.
%
%We are ready to prove the \#P-hardness part of the dichotomy
%by Goldberg et al.~\cite{Goldberg-et-al-2010} (Theorem 1.1) for simple graphs.
%Let $A$ be a real symmetrix $m \times m$ matrix.
%Assuming that $A$ does not satisfy
%the tractability conditions of the dichotomy theorem of Goldberg et al.,
%the problem $\EVAL(A)$ is \#P-hard.
%By Theorem~\ref{thm:EVAL-simp-interp} (with $D = I_m$), $\EVAL(A) \le_{\mathrm T}^{\mathrm P} \EVAL_{\simp}(A)$.
%It follows that $\EVAL_{\simp}(A)$ is \#P-hard.
%
%Hence 
%%Using our proof, 
%the dichotomy theorem by Goldberg et al. %~\cite{Goldberg-et-al-2010}
%can improve to apply to simple graphs.
%\begin{theorem}
%Let $A$ be a real symmetric matrix.
%Then either $\EVAL(A)$ is in polynomial time or $\EVAL_{\simp}(A)$ is \#P-hard
%(a fortiori, $\EVAL(A)$ is \#P-hard).
%
%Moreover, there is a polynomial time algorithm that,
%given the matrix $A$, decides which case of the dichotomy it is. 
%\end{theorem}
%
%%{\color{red} need to trim it down.}
%
%\begin{remark}
%The interpolation argument in Theorem~\ref{thm:EVAL-simp-interp}
%works even if $G$ is a multigraph possibly with multiple loops at any vertex
%in the following sense.
%In Definition~\ref{def:EVAL(A,D)},
%we treat the loops of $G$ as edges.
%We think of them as mapped to the entries $A_{i i}$
%in the evaluation of the partition function $Z_{A, D}$.
%However, we need to slightly change the way we define the graphs $G_n$.
%In addition to $n$-stretching the parallel edges of $G$,
%we also need to $n$-stretch each loop of $G$ (i.e., replacing a loop by
%a closed path of length $n$).
%Now $F$ is the set of parallel edges \emph{and} loops in $G$.
%This way each $G_n = S_n^{(F)}(G)$ for $n \ge 2$ is simple and loopless.
%The rest of the proof goes through.
%In other words, the statement of Theorem~\ref{thm:EVAL-simp-interp}
%extends to a reduction from
%the $\EVAL(A, D)$ problem  that allows input $G$ to have multiloops,
%to the standard problem $\EVAL_{\simp}(A, D)$ not allowing loops.
% %$\EVAL_{\operatorname{multiloops-allowed}}(A, D) \le_{\mathrm T}^{\mathrm P} \EVAL(A, D)$.
%%{\color{red} hideous notation}
%\end{remark}

{\color{red} end of interpolation argument}

{\color{red} sep}

%%%
When $b = 0$, we have $A = a I_\kappa$.
When $b \ne 0$, it is not hard to show that the symmetrix matrix $A = (a - b) I_\kappa + b J_\kappa$
It is easy to show that the matrix $A$ is orthogonally diagonalizable over $\mathbb{R}$, i.e.,
there exist a real orthogonal matrix $S$
and a real diagonal matrix $D = (\lambda_i)_{i = 1}^\kappa$ such that $\widetilde A = S^T D S$.
For the matrix $D = \diag(a - b + \kappa b, a - b, \ldots, a - b)_\kappa$.
Here $\lambda_1 = a - b + \kappa b,\, \lambda_i = a - b$ for $2 \le i \le \kappa$.
If $\lambda_1 = 0$, then $a = b (1 - \kappa)$ which is impossible
since $a, b$ are nonnegative integers, $b \ne 0$ and $\kappa > 3$.

We have $B^{(n)} = A^n = S^T D^t S$.

We can write $B_{i j}^{(n)} = \sum_{\ell = 1}^r a_{i j \ell} \lambda_\ell^n$
by a formal expansion,
for every $n \ge 1$ and some real $a_{i j \ell}$'s
that are dependent on $D$ and $S$, but independent of $n$ and $\lambda_\ell$,
where $1 \le i, j \le m$ and $1 \le \ell \le r$. 

By the formal expansion of the symmetric matrix $B^{(n)}$ above,
we have $a_{i j \ell} = a_{j i \ell}$.

Let $t = |E(G)|$ the number of edges of $G$ counting their multiplicities.

In the evaluation of the Holant function $\PlHolant(\Omega_t)$,
we stratify the edge assignments in $G_n$ as follows.
Denote by  $\kappa = (k_{i j})_{1 \le i \le j \le m}$
a nonnegative tuple with entries indexed by ordered pairs of numbers
and satisfy $\sum_{1 \le i \le j \le m} k_{i j} = t$.

{\color{red} sep}

==> interpolation-hybrid.tex <==
{\color{red} interpolation argument hybrid}

We reduce the problem \#$\kappa$-\textsc{EdgeColoring} over planar ($r$-regular) multigraphs
which is \SHARPP-complete by Theorem \ref{thm:edge_coloring} to simple ($r$-regular) graphs in polynomial time.
Then the statement of the theorem follows.

Assume we can construct an arity $2$ connected simple planar $r$-regular gadget $f$
consisting of only $\AD_{r, \kappa}$ signatures.
By the domain invariance of $\AD_{r, \kappa}$, $f$ is also domain invariant.
Hence its corresponding $\kappa$ by $\kappa$ signature matrix $A = A_f$
has $a_f = a$'s on and $b_f = b$'s off the main diagonal
for some nonnegative integers $a, b$.
In particular, $A$ is symmetric.
We can also write $A = (a - b) I_\kappa + b J_\kappa$.
For any $n \ge 1$, consider an arity $2$ gadget $f_n$
obtained by connecting $f$ sequentially $n$ times
(see Figure~\ref{fig:gadget:k>=r:binary:interpolation}).
Note that the order in which the dangling edges of $f$ are connected to each other
is makes no difference in this construction
because the signature matrix $A$ is symmetric.
Obviously, each gadget $f_n$ for $n \ge 1$ is still planar,
domain invariant and has the signature matrix $A^n$. 
We wish to compute its entries.
Since $J^2 = \kappa J$, we have
\[
A^n = ((a - b) I_\kappa + b J_\kappa)^n = (a - b)^n I_\kappa + \frac{1}{\kappa} \left((a - b + b \kappa)^n - (a - b)^n \right) J_\kappa {\color{red} = \lambda_1^n I_\kappa + \frac{1}{\kappa} (\lambda_1^n - \lambda_2^n ) J_\kappa}.
\]
Here $\lambda_1 = a - b + b \kappa$ and $\lambda_2 = a - b$.
{\color{red}
As a sideline, we note that $\lambda_1, \lambda_2$ are precisely
the eigenvalues of the orthogonally diagonalizable matrix $A$ over $\bbR$
of multiplicities $1$ and $\kappa - 1$ if $b \ne 0$
and $\lambda_1 = \lambda_2 = a$ is
the only eigenvalue of $A = a I_\kappa$ of multiplicity $\kappa$ if $b = 0$.}
Denote $x_n = \frac{1}{\kappa} (a - b + b \kappa)^n + \frac{\kappa - 1}{\kappa} (a - b)^n {\color{red} = \frac{1}{\kappa}\lambda_1^n + \frac{\kappa - 1}{\kappa} \lambda_2^n}$ and $y_n = \frac{1}{\kappa} (a - b + b \kappa)^n - \frac{1}{\kappa}(a - b)^n = {\color{red} \frac{1}{\kappa}\lambda_1^n - \frac{1}{\kappa} \lambda_2^n}$ for $n \ge 1$.
Then $A^n$ has $x_n$'s on and $y_n$'s off the main diagonal for $n \ge 1$.

Assume further that we can satisfy $a \ne b$ and $b \ne 0$.
Then $\lambda_1 = a - b \ne 0$.
Also $\lambda_2 = a - b + b \kappa \ne 0$ as additionally $\kappa \ge 3$. 

Let $\Omega = \Omega(G)$ where $G = (V, E)$ is a multigraph
be an input instance to $\PlHolant(\AD_{r, \kappa})$.
Here every vertex in $V$ is assigned a symmetric signature $\AD_{r, \kappa}$.
Let $F \subseteq E$ be the subset consisting of the edges of $G$
each of which is parallel to at least one other edge (of multiplicity at least two).
For any $n \ge 1$, let $\Omega_n = \Omega(G_n)$ be an instance of $\PlHolant(\AD_{r, \kappa})$ (a signature grid)
obtained by replacing every edge in $G$ by the above gadget $f_n$.
Clearly, for every $n \ge 1$,
the instance $\Omega_n$ (i.e., its underlying graph $G_n$)
remains planar and $r$-regular
and has polynomial size in the size of $\Omega$ and $n$.
Let $m = |F|$; this is precisely the number of the gadgets $f_n$ in $\Omega_n$.
Let $\Omega' = \Omega(G')$ be an signature grid obtained from $\Omega$
by placing the binary \textsc{Equality} signature $=_2$ in the middle of every edge of $G$.
Clearly, $\Holant(\Omega') = \Holant(\Omega)$.

We stratify the assignments on $\Omega$ based on the colors
assigned to the edges of multiplicity at least $2$ of $G$. Then
\[
\Holant(\Omega_n) = \sum_{\ell = 0}^m c_\ell x_n^\ell y_n^{m - \ell} = \sum_{\ell = 0}^m c_\ell (\frac{1}{\kappa}\lambda_1^n - \frac{1}{\kappa} \lambda_2^n)^\ell (\frac{1}{\kappa}\lambda_1^n - \frac{1}{\kappa} \lambda_2^n)^{m - \ell}
\]
where $c_\ell$ is the sum over all assignments of products of evaluations at all vertices
having $\ell$ the same and $n - \ell$ different colors assigned to the edges of $G$.

Expanding out the last sum and rearranging the terms we get
\begin{equation}\label{eq:interpolation-lin-sys-vand} %\label{interpolation-lin-sys-sec4}
\Holant(\Omega_n)
= \sum_{\ell = 0}^m b_\ell (\lambda_1^\ell \lambda_2^{m - \ell})^n.
\end{equation}

This can be viewed as a linear system with the unknowns $b_\ell$ with the rows indexed by $n$. % Vandermonde
The number of unknowns is $m$
which is polynomial in the size of the input instance $\Omega$, since $\kappa$ is a constant.
So the number of unknowns is 
polynomial in the size of the input instance $\Omega$.
The values $\lambda_1^\ell \lambda_2^{m - \ell}$
can all be computed in polynomial time.

We show how to compute the value
\[
\Holant(\Omega') = \sum_{\ell = 0}^m b_\ell,
\]
from the values $\Holant(\Omega_n)$ where $n \ge 1$ in polynomial time.
The coefficient matrix of the linear system (\ref{eq:interpolation-lin-sys-vand})
 is Vandermonde.
However, it might not be of full rank
because the coefficients $\lambda_1^\ell \lambda_2^{m - \ell}$
do not have to be pairwise distinct, and therefore
it can have repeating columns.
Nevertheless, when there are two repeating columns we replace
the corresponding unknowns $b_{\ell}$ and $b_{\ell'}$
with their sum as a new variable; we repeat this replacement procedure until
there are no repeating columns.
Since $\lambda_1,\, \lambda_2 \ne 0$,
after the replacement,
 we have a Vandermonde system of full rank.
% after all such combinations.
Therefore we can solve this modified linear system
in polynomial time and find the desired value $\Holant(\Omega) = \Holant(\Omega') = \sum_{\ell = 0}^m b_\ell$.




==> triangledef.tex <==
%%% BEGIN: define new arrow tip ``new open triangle 60''
%%% see bug: http://sourceforge.net/tracker/index.php?func=detail&aid=3609043&group_id=142562&atid=752792
\makeatletter
\pgfarrowsdeclare{new open triangle 60}{new open triangle 60}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=7.29\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}6
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
    \pgfsetfillcolor{white}
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}
%%% END: define new arrow tip ``new open triangle 60''

